Unified Guidance for Geometry-Conditioned Molecular Generation

Effectively designing molecular geometries is essential to advancing pharmaceutical innovations, a domain, which has experienced great attention through the success of generative models and, in particular, diffusion models. However, current molecular diffusion models are tailored towards a specific downstream task and lack adaptability. We introduce UniGuide, a framework for controlled geometric guidance of unconditional diffusion models that allows flexible conditioning during inference without the requirement of extra training or networks. We show how applications such as structure-based, fragment-based, and ligand-based drug design are formulated in the UniGuide framework and demonstrate on-par or superior performance compared to specialised models. Offering a more versatile approach, UniGuide has the potential to streamline the development of molecular generative models, allowing them to be readily used in diverse application scenarios.

==> chapters/wraps/app_sbdd_qual.tex <==
\begin{figure}[]
    \includegraphics[width=0.6\linewidth]{figures/sbdd_qualitative}
        %\vspace{-2em}
    \caption{Qualitative example of a test protein pocket (6c0b) from the Binding MOAD dataset. We show the reference ligand (grey) and samples generated by \ours\ (blue).} 
    \label{fig:sbdd_qualitative}
\end{figure}
